Approximate Cross-validated Mean Estimates for Bayesian Hierarchical Regression Models

We introduce a novel procedure for obtaining cross-validated predictive estimates for Bayesian hierarchical regression models (BHRMs). Bayesian hierarchical models are popular for their ability to model complex dependence structures and provide probabilistic uncertainty estimates, but can be computationally expensive to run. Cross-validation (CV) is therefore not a common practice to evaluate the predictive performance of BHRMs. Our method circumvents the need to re-run computationally costly estimation methods for each cross-validation fold and makes CV more feasible for large BHRMs. By conditioning on the variance-covariance parameters, we shift the CV problem from probability-based sampling to a simple and familiar optimization problem. In many cases, this produces estimates which are equivalent to full CV. We provide theoretical results and demonstrate its efficacy on publicly available data and in simulations.

==> preamble.tex <==

\usepackage[sort]{natbib}
\bibpunct[, ]{(}{)}{;}{a}{,}{,}
\renewcommand\bibfont{\fontsize{10}{12}\selectfont}%

\usepackage{amsmath}
\usepackage{physics}
\usepackage{float}
%\usepackage[notablist,heads,tablesfirst]{endfloat}
\usepackage{soul} % user-provided, for strike throughs
\usepackage{xcolor} % for textcolor
%\pdfminorversion=4
% NOTE: To produce blinded version, replace "0" with "1" below.
\newcommand{\blind}{0}

% DON'T change margins - should be 1 inch all around.
\addtolength{\oddsidemargin}{-.5in}%
\addtolength{\evensidemargin}{-.5in}%
\addtolength{\textwidth}{1in}%
\addtolength{\textheight}{1.3in}%
\addtolength{\topmargin}{-.8in}%

\newcommand{\edit}[1]{\textcolor{black}{#1}}
\newcommand{\newedit}[1]{\textcolor{purple}{#1}}
\newcommand{\ereft}[1]{Equation (\ref{#1})}


\usepackage{url}            % simple URL typesetting
\usepackage{booktabs, makecell, multirow, tabularx}       % professional-quality tables
\usepackage{mathtools}  % coloneqq
\usepackage{nameref, hyperref, cleveref}
\usepackage{bbm}
\usepackage{bm}
\usepackage{amsthm}
\theoremstyle{plain}% Theorem-like structures provided by amsthm.sty
\newtheorem{theorem}{Theorem}[section]
\newtheorem{lemma}[theorem]{Lemma}
\newtheorem{corollary}[theorem]{Corollary}
\newtheorem{proposition}[theorem]{Proposition}

\theoremstyle{definition}
\newtheorem{definition}[theorem]{Definition}
\newtheorem{example}[theorem]{Example}

\theoremstyle{remark}
\newtheorem{remark}{Remark}
\newtheorem{notation}{Notation}

% The \author macro works with any number of authors. There are two commands
% used to separate the names and addresses of multiple authors: \And and \AND.
%
% Using \And between authors leaves it to LaTeX to determine where to break the
% lines. Using \AND forces a line break at that point. So, if LaTeX puts 3 of 4
% authors names on the first line, and the last on the second line, try using
% \AND instead of \And before the third author name.

\newcommand{\RR}{I\!\!R} %real numbers

% placeholder symbol for the number of non-zero entries in a row of X




\newcommand{\bigo}[1]{\mathcal{O}\left( #1 \right)}
\newcommand{\bigop}[1]{\mathcal{O}_P\left( #1 \right)}

\DeclareMathOperator*{\argmax}{argmax}
\newcommand{\parens}[1]{\left(#1 \right)}

\DeclareMathAlphabet{\mathpzc}{OT1}{pzc}{m}{it}
